Two Slits Interference Is Compatible with Particles' Trajectories

We propose a simple numerical experiment of two slits interference of particles. It disproves the popular belief that such an interference is incompatible with a knowledge which slit each particle came through or, more generally, ``quantum particles could not have trajectories''. Our model is an illustration to the contextual interpretation of quantum probabilities.

==> mydef.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       $Id: mydef.tex,v 1.20 2001/05/24 15:29:33 kisilv Exp kisilv $    
%
%  File mydef.tex
%
\typeout{This is MyDef macros file}
\makeatletter
\def\ifundefined#1{\expandafter\ifx\csname#1\endcsname\relax}
\hyphenation{di-men-sio-nal}
\providecommand{\comment}[1]{}
\def\smnegskip{\mskip-0.6\thinmuskip}
\usepackage{amsfonts}
\providecommand{\tthdump}[1]{#1}
\tthdump{\newlength{\curmathsize}}
%
%   Objects
%
\newcommand{\algebra}[1]{\ensuremath{\mathfrak{#1}}}
\newcommand{\Heisen}[1]{{\ensuremath{\mathbb{H}^{#1}}}}
\newcommand{\hHeisen}[1]{\ensuremath{\widehat{\mathbb {H}}^{#1}}}
\newcommand{\Cliff}[2][\comment]{{\ensuremath{%
\mathcal{C}\kern-0.18em\ell(#1,#2)}}}
%\newcommand{\Cliff}[2][\comment]{\ensuremath{\mathbf{Cl}(#1,#2)}}
\newcommand{\object}[2][\,]{\ensuremath{\mathrm{#2}#1}}
\newcommand{\Space}[3][]{\ensuremath{\mathbb{#2}^{#3}_{#1}{}}}
\newcommand{\such}{\,\mid\,}
\newcommand{\Jacobian}[1]{\ensuremath{\mathcal{J}(#1)}}
\newcommand{\FSpace}[3][]{\ensuremath{ #2_{#3}^{#1}{}}}
\newcommand{\Quater}{\ensuremath{\mathcal{H}}}
\newcommand{\bos}{\mathcal{B}}
\ifundefined{qed}
    \DeclareMathSymbol{\qed}{0}{AMSa}{"03}
\fi
\newcommand{\SL}[1][2]{\ensuremath{\FSpace{SL}{#1}(\Space{R}{})}}
%
%  Unary operations
%
\newcommand{\fourier}[1]{\ensuremath{\mathcal{F}^{#1}{}}}
\newcommand{\bra}[1]{\ensuremath{\left\langle#1\right|}}
\newcommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\newcommand{\Cplus}{\ensuremath{C^{+}}}
\newcommand{\Cstar}{\ensuremath{C^{*}}}
\newcommand{\onvol}{^{+}}
\newcommand{\spec}{\ensuremath{\mathbf{sp}}}
\newcommand{\sr}{\ensuremath{\mathbf{r}}\,}
\newcommand{\kernel}{\ensuremath{\mathbf{ker}}\,}
\newcommand{\ad}{\ensuremath{\mathbf{ad}}\,}
\newcommand{\diag}{\mathop {\operator@font diag}\nolimits}
\newcommand{\norm}[2][\relax]{\left\|#2\right\|\ifx#1\relax\else_{#1}\fi}
\newcommand{\modulus}[2][\relax]{\left| #2 \right|\ifx#1\relax\else_{#1}\fi}
\newcommand{\oper}[1]{\mathcal{#1}}
%
%  Binary operations%
\newcommand{\scalar}[3][\relax]{\left\langle #2,#3 
        \right\rangle\ifx#1\relax\else_{#1}\fi}
\newcommand{\intersect}[2]{\left.#1\right|_{#2}}
\newcommand{\relstack}[2]{{\mathrel {\mathop {#1}\limits _{#2}}}}
%
%
%
\providecommand{\eqref}[1]{\textup{(\ref{#1})}}
\newcommand{\eqnright}[1]{\qquad\qquad  #1}
\newcommand{\person}[1]{\textsc{#1}}
%
%  WWW commands
%
\providecommand{\href}[2]{#2}
\iftth
  \special{html:<BODY BGCOLOR=ffffff>}
  \newcommand{\MR}[1]{%
\textbf{MR}~\special{html:<a href="http://www.ams.org/mathscinet-getitem?mr=#1">\#~#1</a>}}
  \newcommand{\Zbl}[1]{%
\textbf{Zbl}~\special{html:<a href="http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete">\#~#1</a>}}
\else
  \newcommand{\MR}[1]{\textbf{MR}~\href{http://www.ams.org/mathscinet-getitem?mr=#1}{\#~#1}}
  \newcommand{\Zbl}[1]{\textbf{Zbl}~\href{http://www.emis.de:80/cgi-bin/zmen/ZMATH/en/zmathf.html?first=1&maxdocs=3&type=html&an=#1&format=complete}{\#~#1}}
\fi

\newcommand{\eprint}[2]{E-print: \href{#1}{\texttt{#2}}}
\newcommand{\mailto}[1]{\href{mailto:#1}{\texttt{#1}}}
\newcommand{\urltt}[1]{\href{#1}{\texttt{#1}}}
%
\makeatother
\endinput

